Design and Analysis of Pairing-Friendly Elliptic Curves for Cryptographic Primitives

Elliptic curve cryptography (ECC) is a remarkable mathematical tool that offers the same level of security as traditional public-key cryptography (PKC) with a significantly smaller key size and lower computational requirements. The use of pairing on elliptic curves has emerged as a vibrant field of research that provides enhanced security measures for the next generation of cryptographic systems. This thesis explores using ECC and Pairing-Based Cryptosystems (PBC) as effective mathematical tools for achieving high-security levels with minimal key size and computation cost. Specifically, the research aims to analyze Pairing-Friendly Elliptic Curves (PF-EC) and their practicality in resource-constrained environments. It proposes solutions to some of the limitations of existing applications of pairing-based cryptography. The thesis begins by presenting a comprehensive framework for constructing PF-EC and evaluating the practical security of several families of pairing-friendly curves. The study then explores the limitations of Identity-Based Encryption (IBE), a recognized application of pairing-based cryptography. It proposes mechanisms to address issues such as key escrow, secure key issuing, user slandering, and key abusing problems. The proposed solutions include an Escrow-Free Identity-Based Encryption (EF-IBE) scheme secured against confidentiality and an Escrow-Free Identity-Based Signature (EF-IBS) scheme that is forgeable and secure.

==> endmatter/append.tex <==
\chapter*{Appendices}


\begin{figure}
  \centering
  \includegraphics[height=8cm]{figures/append1.eps}
 % \caption{Communication cost comparison of proposed IBAAKA scheme with other schemes}
\label{figappend1}
\end{figure}

==> frontmatter/JNUheader.tex <==
\begin{minipage}[l]{0.15\textwidth}%
    % \noindent
    \includegraphics[width=1\textwidth]{figures/JNU_logo_colored.pdf}
\end{minipage}%
\hfill
\begin{minipage}[l]{0.85\textwidth}%
    \begin{center}
     {
     %{\hindi कंप्यूटर एवम् पद्धति विज्ञान संस्थान }
     \par
     \large School of Computer \& Systems Sciences  \par\vspace{5pt}
    % {\hindiB जवाहरलाल नेहरू विश्वविद्यालय}
     \par
     \uppercase{\large \scshape\bfseries Jawaharlal Nehru University \par}
     %{\hindiB नई दिल्ली}
     /
     \large New Delhi - 110067 \par
      }
      \vspace{0.3cm}
    \end{center}
\end{minipage}%
\hrule



==> frontmatter/abstract.tex <==
% the abstract
Elliptic curve cryptography (ECC) is a remarkable mathematical tool that offers the same level of security as traditional public-key cryptography (PKC) with a significantly smaller key size and lower computational requirements. The use of pairing on elliptic curves has emerged as a vibrant field of research that provides enhanced security measures for the next generation of cryptographic systems.

This thesis explores using ECC and Pairing-Based Cryptosystems (PBC) as effective mathematical tools for achieving high-security levels with minimal key size and computation cost. Specifically, the research aims to analyze Pairing-Friendly Elliptic Curves (PF-EC) and their practicality in resource-constrained environments. It proposes solutions to some of the limitations of existing applications of pairing-based cryptography.

The thesis begins by presenting a comprehensive framework for constructing PF-EC and evaluating the practical security of several families of pairing-friendly curves. The study then explores the limitations of Identity-Based Encryption (IBE), a recognized application of pairing-based cryptography. It proposes mechanisms to address issues such as key escrow, secure key issuing, user slandering, and key abusing problems. The proposed solutions include an Escrow-Free Identity-Based Encryption (EF-IBE) scheme secured against confidentiality and an Escrow-Free Identity-Based Signature (EF-IBS) scheme that is forgeable and secure.

Next, the thesis examines the feasibility of Internet-Voting Systems (IVS) and identifies user anonymity and ballot integrity during distribution as the main issues hindering their practical implementation. To address these challenges, the thesis proposes two cryptographic primitives secured under the Computational Diffie-Hellman Problem (CDHP) and the Random Oracle Model (ROM) and implements an End-to-End Verifiable Internet Voting (E2E-VIV) system with batch verifiability using one of the proposed cryptographic protocols.

The research also studies the security issues associated with data outsourcing in the cloud and proposes an Identity-Based Blind Signature with a Message Recovery (IDBS-MR) scheme to implement a privacy-preserving data outsourcing mechanism that audits the integrity of stored data for resource-limited devices in cloud computing.

Furthermore, the thesis proposes two kinds of Escrow-Free Identity-Based Signcryption (EF-IDSC) schemes and implements a secure peer-to-peer video-on-demand (P2P-VoD) streaming system and a secure cloud-assisted health care system that achieves public verifiability based on the identity-based aggregated signcryption (IDASC) scheme.

Finally, the research focuses on realizing an authenticated (anonymous) key agreement protocol in energy-constrained settings and proposes two identity-based authenticated key agreement protocols to obtain a secure session key in health care. The first protocol is a One-Round Three-Party Authenticated Identity-Based Key Agreement Protocol (OR-3PID-KAP). In contrast, the second is an Identity-Based Anonymous Authentication and Key Agreement (IBAAKA) protocol for Wireless Body Area Networks (WBANs) in the cloud-assisted environment, which achieves mutual authentication and user anonymity.

The thesis concludes by summarizing the main findings and proposing directions for future work, including a discussion of a data-sharing scheme based on the Hyperledger Fabric (HF) in the context of the COVID-19 crisis. The research in this thesis provides a step-by-step guide to the design and implementation of efficient and secure cryptosystems using ECC and PBC.

==> frontmatter/dedication.tex <==
% dedication text
\textit{Dedicated to my father...}

==> frontmatter/listofpublications.tex <==
\textbf{List of communicated manuscripts}
\vspace{5mm}
\begin{enumerate}
     \item \textbf{Mahender Kumar}, and Satish Chand. “An Identity-Based Privacy-Preserving with Integrity   Auditing for Resource-Constrained Devices in Cloud Storage” (Communicated). 
    \item \textbf{Mahender Kumar}, and Satish Chand. “MedHypChain: A Patient-Centered Interoperability Hyperledger-Based Medical Healthcare System: Regulation in COVID-19 Pandemic” (Communicated). 
    \item \textbf{Mahender Kumar}, and Satish Chand. “Pairing-Friendly Elliptic Curves: Classification, Recent Attacks and Their Security ” (Communicated).
    \item \textbf{Mahender Kumar}, and Satish Chand. “Pairing for Greenhorn: Survey and Future Perspective ” (Communicated).
    \item \textbf{Mahender Kumar}, and Ruby Rani. “SAI-BA-IoMT: Secure AI-Based Blockchain-Assisted Internet of Medical Things Tool to Moderate the Outbreak of COVID-19 Crisis” (Communicated).
    \item \textbf{Mahender Kumar}, and Satish Chand. “A flexible and efficient end-to-end anonymous authentication for heterogeneous platform in multi-access edge computing” (Communicated).
\end{enumerate}
\vspace{10mm}
\textbf{List of Journals} 
\vspace{5mm}
\begin{enumerate}
   \item \textbf{Mahender Kumar}, and Satish Chand. \href{https://ieeexplore.ieee.org/document/9131770}{\textit{“A Secure and Efficient Cloud-Centric Internet of Medical Things-Enabled Smart Healthcare System with Public Verifiability”}}, IEEE Internet of Things Journals. doi: 10.1109/JIOT.2020.3006523. (\textbf{SCIE, IF: 9.94}) \cite{Kumar2020IoMT}
    \item \textbf{Mahender Kumar}, and Satish Chand. “A Secure and Efficient Identity-Based Signature Scheme against Mali-cious-but-Passive Private Key Generator” Frontiers of Information Technology \& Electronic Engineering, Springer. (Revision) (\textbf{SCIE, IF: 1.6}) 
    \item \textbf{Mahender Kumar}, and Satish Chand. \href{https://ieeexplore.ieee.org/document/9099043}{\textit{"A Lightweight Cloud-Assisted Identity-Based Anonymous Authentication and Key Agreement Protocol for Secure Wireless Body Area Network."}}, IEEE Systems Journal (2020), doi: 10.1109/JSYST.2020.2990749. (\textbf{SCIE, IF: 4.462}) \cite{kumar2020lightweight}
    \item \textbf{Mahender Kumar}, Satish Chand, and C. P. Katti. \href{https://ieeexplore.ieee.org/abstract/document/8977363}{\textit{"A Secure End-to-End Verifiable Internet-Voting System Using Identity-Based Blind Signature."}}, IEEE Systems Journal (2020) 14.2 (2020): 2032-2041. (\textbf{SCIE, IF: 4.642}) \cite{kumar2020secure}
    \item \textbf{Mahender Kumar}, and Satish Chand. \href{https://link.springer.com/article/10.1007/s11042-019-08330-5}{"\textit{SecP2PVoD: a secure peer-to-peer video-on-demand system against pollution attack and untrusted service provider}."}, Multimedia Tools and Applications 79.9 (2020): 6163-6190. (\textbf{SCIE, IF: 2.101}) \cite{kumar2020secp2pvod}
    \item \textbf{Mahender Kumar}, Satish Chand. \href{https://link.springer.com/article/10.1007/s11277-020-07520-x}{"\textit{Escrow-Less Identity-Based Signature Scheme with Outsourced Protection in Cloud Computing}"}. Wireless Pers Commun, Springer (2020).\\ https://doi.org/10.1007/s11277-020-07520-x (\textbf{SCIE, IF: 1.06}) \cite{kumar2020escrow}
    \item \textbf{Mahender Kumar} and Satish Chand. \href{https://link.springer.com/article/10.1007/s11042-019-7155-x}{"\textit{ESKI-IBE: Efficient and secure key issuing identity-based encryption with cloud privacy centers.}"}, Multimedia Tools and Applications, Springer, 78.14 (2019): 19753-19786. (\textbf{SCIE, IF: 2.101}) \cite{kumar2019eski}
    \item \textbf{Mahender Kumar}, \href{https://eprint.iacr.org/2020/936}{"\textit{Cryptanalysis and Improvement of Anonymous Authentication for Wireless Body Area Networks with Provable Security}"} Cryptology ePrint Archive: Report 2020/936. \cite{kumar2020cryptanalysis}
    \item \textbf{Mahender Kumar}, C. P. Katti, and P. C. Saxena. \href{https://serialsjournals.com/abstract/94051_14-mahender_kumar.pdf}{”\textit{A new blind signature scheme using identity-based technique}”} Int. J. Control Theor. Appl 10.15 (2017): 115-124. \cite{kumar2017new}
    \item \textbf{Mahender Kumar}, C. P. Katti, and P. C. Saxena. \href{https://www.semanticscholar.org/paper/An-Identity-based-Blind-Signature-Approach-for-Kumar-Katti/60170ab0ae6720f965597040c70c24472fec6707}{”\textit{An Identity-based Blind Signature Approach for E-voting System}”}, International Journal of Modern Education and Computer Science 9.10 (2017): 47. \cite{kumar2017identity}
    \item \textbf{Mahender Kumar} and C. P. Katti, \href{https://www.semanticscholar.org/paper/An-efficient-ID-based-partially-blind-signature-and-Kumar-Katti/b4567352d36d857e7c969ccb9910102477f1bc57}{“\textit{An efficient ID-based partially blind signature scheme and application in electronic-cash payment system}”}, Accent. Trans. Inf. Secur., vol. 2, no. 6 pp. 36–42, Dec. 2016. \cite{kumar2016efficient}
\end{enumerate}

\textbf{List of Conferences/Workshops}
\begin{enumerate}
    \item \textbf{Mahender Kumar}, and Satish Chand. \href{https://link.springer.com/chapter/10.1007/978-3-030-42921-8_24}{"\textit{A Pairing-Less Identity-Based Blind Signature with Message Recovery Scheme for Cloud-Assisted Services.}"}, International Conference on Information Security and Cryptology. Springer, Cham, 2019. \cite{kumar2020pairing}
   \item \textbf{Mahender Kumar}, and P. C. Saxena. \href{https://link.springer.com/chapter/10.1007/978-981-13-3804-5_31}{”\textit{Pairing-Free Authenticated Identity-Based Two-Party Key Agreement Protocol for Resource-Constraint Devices}”} International conference on Futuristic trend in network and communication technologies, CCIS, Springer, 9-10 Feb 2018. \cite{kumar2019PF}
    \item \textbf{M. Kumar}, C.P. Katti, and P. C. Saxena, “\href{https://link.springer.com/chapter/10.1007/978-3-319-72598-7_3}{\textit{A Secure Anonymous E-Voting System Using Identity-Based Blind Signature Scheme}},” in International Conference on Information Systems Security, LNCS, Springer 2017, pp. 29–49. \cite{kumar2017secure}
     \item \textbf{Mahender Kumar}, and P. C. Saxena. \href{https://papers.ssrn.com/sol3/papers.cfm?abstract_id=3166740}{”\textit{One-Round Authenticated Identity-Based Tri-Partite Key Agreement Protocol for Internet of Things Based Sensors}”}, 3rd International Conference on Internet of Things and Connected Technologies (ICIoTCT), 26-28 March 2018 \cite{kumar2018one}
   \item \textbf{Mahender. Kumar} C. P. Katti and P.C. Saxena, “\href{https://link.springer.com/chapter/10.1007/978-3-319-73423-1_7}{\textit{An Untraceable Identity-Based Blind Signature Scheme without Pairing for E-cash Payment System}},” in International Conference on Ubiquitous Communication and Network Computing, 2017. \cite{kumar2017untraceable}
   \item \textbf{Mahender Kumar}, C. P. . Kumar and S. P.C., “A new blind signature scheme using identity-based technique,” 2nd International Conference on Sustainable Computing Techniques in Engineering, Science and Management (SCESM 2017), 27- 28 Jan 2017. 
   \item  \textbf{Mahender Kumar}, C.P. Katti, “An Efficient ID-Based Partially Blind Signature Scheme and Application in Electronic-Cash Payment System”, National Workshop for Cryptography 2016, JNNCE, Shimogga, 2016.
\end{enumerate}

\textbf{Books/Chapters}
\begin{enumerate}
    \item \textbf{Mahender Kumar}, \href{https://link.springer.com/chapter/10.1007/978-3-662-57277-1_18}{”\textit{AOR-ID-KAP: An Authenticated One-Round Identity-Based Key Agreement Protocol for Wireless Sensor Network}”}, Computational Intelligence in Sensor Networks, published in Studies in computational intelligence, Springer, 2019. \cite{kumar2019aor}
\end{enumerate}


==> frontmatter/listofsymbol.tex <==
\begin{longtable}{ll}
    $K$ &	Field\\
$\overline{K}$ &	Algebraic closure of K \\
$k$ &	Embedding degree\\
$\mathbb{F}_p$ &	Finite field of prime $p$\\
$\mathbb{F}_{p^k}$ &	Field extension of $p^k$ \\
$\mathbb{Q}$ &	Rational number  \\
$\mathbb{Z} $ &	Integer \\
$p$	& Field size \\
$r$ &	Prime order of subgroup \\
$E(\mathbb{F}_p)$ &	Elliptic curve over field of prime p\\
$\#E(\mathbb{F}_p)$ &	Order of elliptic curve over field of prime p\\
$\rho$	& Denotes closeness of size of subgroup r and size of field p\\
$d$ &	Integer to represent a twist in a curve\\
$E/K$ &	Elliptic curve over field $K$ \\
$t$ &	Trace of fohrehenus \\
$E(\mathbb{F}_{p^k})[r]$ &	group of r-torsion points of E defined over $\mathbb{F}_{p^k}$\\
$x|y$ &	x is divisible by y\\
$x\subset y$ &	x is subset of y\\
$<r,p,t>$ &	Parameter set to present the pairing-friendly curve \\
$<r(x_0),p(x_0),t(x_0)>$ & 	Parameter set to present the family of curve\\
$\Phi_k (x)$ &	$k^{th}$ cyclotomic polynomial\\
$\Phi_l(u(x))$ &	cyclotomic polynomials on any polynomial u(x)\\
$D$ &	Discriminant \\
$\zeta_k$	& $K^{th}$ root of unity\\
$L_N[l:c]$	& L notation \\
$degf$ &	Degree of f\\
$\mu$ &	Slope on curve\\
$e_W$ &	Weil pairing\\
$\tau$ &	Tate pairing \\
$f_P$ &	Rational function on point P in elliptic curve \\
$ \in $ &	Belong to\\
$ \notin $ & Not belong to\\
$\Phi :  E \rightarrow E $ & Distorted map from E to itself\\
$\epsilon $ &	Negligible function \\ 
$k \in \mathbb{Z}_q$ & 	Security parameter\\
$\mathbb{G}_1 $ &	Additive cyclic group on elliptic curve\\
$\mathbb{G}_2$ &	Multiplicative cyclic groups on elliptic curve \\
$q$ & 	Order of group $\mathbb{G}_1$ and $\mathbb{G}_2$\\
$P$ &	Generator of $\mathbb{G}_1$\\
$e: \mathbb{G}_1  \times \mathbb{G}_1 \rightarrow \mathbb{G}_2$ &	Bilinear mapping\\
$s_0,P_0$ & 	Master secret key and public key of KGC/PKG\\
$s_i,P_i$ & 	Secret key and public key of $i^{th}$ CPC\\
$Y$ &	System public key\\
$pp$ & Public parameter\\
$M,C \in \{0,1\}^n$ & Message and ciphertext of  length n \\
$ID_X \in \{0,1\}^n$ & Unique identification of entity X\\
$d_X$ & 	Actual private key of entity X \\
$Adv$ &	Adversary \\
$F$ & Forger \\
$Ch$ &	Challenger\\
$B$ &	Simulator that helps adversary respectively \\
$ID^{ch}$ and $C^{ch}$ &	Challenged identity and ciphertext \\
$\oplus$ &	X-OR operation \\
IBC/E/S &	Identity-based cryptosystem/Encryption/Signature\\
ESKI &	Efficient and Secure key issuing  \\
ESKI-IBE &	Identity-based encryption based on ESKI scheme\\
KGC/CPC & Key Generation Center/ Cloud Privacy Center\\
IND-ID-CPA	& Indistinguishability under chosen-plaintext attack model for IBE \\
IND-ID-CCA &	Indistinguishability under chosen-ciphertext attack model for IBE\\
BasicESKI-IBE &	ESKI-IBE scheme is secure against IND-ID-CPA\\
FullESKI-IBE &	ESKI-IBE scheme is secure against IND-ID-CCA\\
$<d_X,R_X>$ &	Private key of entity X in E2E-VIV system  \\
$R$ &	Pseudonym public key of voter\\
$a,b,c,d,e,f$ &	Pseudonym private key of voter\\
$absc(P)$ &	x coordinate of point P on elliptic curve\\
$\sigma$ &	Signature on message\\
$BB=<s,R,h>$ &	Pseudonym Certificate or blank ballot\\
$C_{name}$ &	Candidate name that a voter supports\\
$Bt$	& Ballot\\
$Rcpt/S_{Rcpt}$ &	Acknowledgement/ signed acknowledgment by ECA\\
$n_c$ &	Random number for the uniqueness in each Rcpt\\
$List^{RV}$ &	Biometric details of registered voters \\
$List^{RC}$ &	Biometric details of registered candidates \\
$List^{VV}$ &	Biometric details of registered voters to whom ballot has been issued\\
$List^B$ &	Valid/invalid ballots of registered voters\\
$List^{VB}$ &	Valid ballot list of registered voters\\
$List^{IB}$	& Invalid ballots list of registered voters\\
$d \in \{0,1\}^{l2}$ & Data block of any length l2\\
$F_{ID}$ &	File name identifier\\
$b_1$, $b_2$ &	Blinded data block\\
$I$ &	Data index\\
|| &	Concatenation of two strings \\
$_{l1}^{l}|u|$	& First l1 bit of string u from left\\
$|u|_{l2}^R$ & First l2 bit of string u from right\\
$p2p_{sk}$ &	One time session key between two peers\\
$T$ &	Timestamp \\
$chk$ & data	chunk\\
$ID_{BMS}^j$, $d_{BMS}^j$ & Identity and private key of $j^{th}$ BMS\\
$m_{i,j}$	& $i^{th}$ Message of $j^{th}$ BMS\\
$C_{aggr,j}$ &	Aggregated ciphertext on $j^{th}$ BMS \\
$C_{PAD}$ &	Aggregated ciphertext on PAD \\
LN &	Leaf node\\ 
CS & 	Cloud server\\
TN &	Target node\\
NM &	Network manager \\
RN &	Root node \\
IBAAKA &	Identity-based anonymous authentication and key agreement\\
$S_{CS}$ &	Long term private ley of CS\\
$s_{LN}$ &	Long term private key of LN\\
$H_i (i=1,2,.,7)$ &	Cryptographic hash functions \\


\end{longtable}

==> frontmatter/thanks.tex <==
% the acknowledgments section
I am grateful to many people who helped me throughout my PhD journey. It would not have been possible to achieve this magnitude without the guidance of my supervisor, Professor Satish Chand, and ex-supervisor, Professor C.P. Katti.

I want to thank Emeritus Professor Prem Chandra Saxena, who has always nurtured me with moral support.

I want to thank each Dean of the SC\&SS during my PhD journey for their valuable support. Besides, I would like thanks to the SC\&SS office staff for their behaviour.

I could not forget to acknowledge the atmosphere and support of Dr B. R. Ambedkar Central Library and its staff, where a significant portion of the thesis has been accomplished.

I would also mention the 37 rejections for the first acceptance that made me more determined and sharpened my tendency. I would especially like to give a notable technical contribution to anonymous reviewers for their honest comments, who corrected me, where I was inaccurate. 

I appreciate the scholarship provided by the Council of Scientific and Industrial Research (CSIR); without their financial support, I could not continue this journey.

I pay my thanks to Ms Ruby, who has been encouraging me from the beginning of the journey to date and stood with me in my ups and downs. 

I want to thank my mother, father, brother, sisters, sister-in-law, and kids in the family who contributed to the journey by providing me with ample space, leisure, and patience.

I also extend my gratitude to all my friends and colleagues who directly or indirectly helped in one or the other way.  
 
